Neural Mesh Flow: 3D Manifold Mesh Generation via Diffeomorphic Flows

Meshes are important representations of physical 3D entities in the virtual world. Applications like rendering, simulations and 3D printing require meshes to be manifold so that they can interact with the world like the real objects they represent. Prior methods generate meshes with great geometric accuracy but poor manifoldness. In this work, we propose Neural Mesh Flow (NMF) to generate two-manifold meshes for genus-0 shapes. Specifically, NMF is a shape auto-encoder consisting of several Neural Ordinary Differential Equation (NODE)[1] blocks that learn accurate mesh geometry by progressively deforming a spherical mesh. Training NMF is simpler compared to state-of-the-art methods since it does not require any explicit mesh-based regularization. Our experiments demonstrate that NMF facilitates several applications such as single-view mesh reconstruction, global shape parameterization, texture mapping, shape deformation and correspondence. Importantly, we demonstrate that manifold meshes generated using NMF are better-suited for physically-based rendering and simulation. Code and data are released.

==> _OLD_experiments.tex <==
% \section{Experiments}

% \subsection{Shape Auto Encoding}
% For the task of shape generation from a point cloud $X$, we first sample 1024 points and obtain the shape embedding $z$ using the PointNet encoder $Q_{\phi}(z|X)$. Then we take a sphere consisting of equally spaced 1024 points $X_0$ and pass thorough $\mathcal{F}_{\Theta|z}$ and back-propagate based on the loss described in eq. \ref{totalloss}. Since the topology is maintained, in order to generate a high-resolution mesh, we take a spherical mesh $S^*$ consisting of ~2500 vertices and pass these vertices along with the shape embedding $z$ to NMF. Since the output point set has the same topology as $S^*$, we simply use the adjacency information of corresponding vertices in $S^*$ to obtain the final mesh.

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Images/AE/ae-chair-crop.pdf}
%     \caption{Shape Auto Encoding Results}
%     \label{fig:my_label}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Images/AE/ae-bench-crop.pdf}
%     \caption{Shape Auto Encoding Results}
%     \label{fig:my_label}
% \end{figure}


% \subsubsection{Generalization}

% \subsubsection{Interpolation}

% \begin{figure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/chair-chair/1.png}
% %   \caption{1a}
%   \label{fig:sfig1}
% \end{subfigure}%
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/chair-chair/3.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/chair-chair/4.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/chair-chair/5.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/chair-chair/7.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/chair-chair/10.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}

% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/car-speaker/1.png}
% %   \caption{1a}
%   \label{fig:sfig1}
% \end{subfigure}%
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/car-speaker/3.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/car-speaker/5.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/car-speaker/7.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/car-speaker/9.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/car-speaker/11.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}

% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/table-lamp/1.png}
% %   \caption{1a}
%   \label{fig:sfig1}
% \end{subfigure}%
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/table-lamp/3.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/table-lamp/5.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/table-lamp/7.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/table-lamp/9.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/table-lamp/11.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}

% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/plane-bench/1.png}
% %   \caption{1a}
%   \label{fig:sfig1}
% \end{subfigure}%
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/plane-bench/3.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/plane-bench/5.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/plane-bench/7.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/plane-bench/9.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.16\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/Interpolation/plane-bench/11.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}

% \caption{Interpolation}
% \label{fig:fig}
% \end{figure}

% \begin{figure}
% \begin{subfigure}{\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/semantic/table-chair-org.png}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/semantic/table-chair-tran.png}
% %   \caption{1b}
%   \label{fig:sfig2}
%   \end{subfigure}
% \caption{Semantic correspondence}
% \label{fig:fig}
% \end{figure}

% \begin{figure}
% \begin{subfigure}{.4\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/checker.jpg}
% %   \caption{1b}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/texture.png}
% %   \caption{1b}
%   \label{fig:sfig2}
%   \end{subfigure}
% \caption{Texture Mapping}
% \label{fig:fig}
% \end{figure}

% \begin{figure}

%     \centering
%     \includegraphics{}
%     \caption{Caption}
%     \label{\begin{subfigure}
      
%     \end{subfigure}}
% \end{figure}

% \subsubsection{Consistent Correspondence}

% \subsection{Single View Reconstruction}
% \begin{figure}
%   \centering
%   \includegraphics[width=\linewidth]{Images/svr.pdf}
% %   \captio
% \caption{Single View Reconstruction}
% \label{fig:fig}
% \end{figure}
% \subsection{Shape Parameterization}

% \subsection{Comparison with Implicit Representation methods}

% \subsection{Training}


\section{Results}

In this section we show qualitative and quantitative results on the task of auto-encoding and single view reconstruction of 3D shapes with comparison against several state of the art baselines. In addition to these tasks, we also demonstrate several additional features and applications of our approach including latent space interpolation texture mapping, consistent correspondence and shape deformations in the supplementary material.

\vspace{-0.2cm}
\paragraph{Data} We evaluate our approach on the ShapeNet Core dataset \cite{shapenet}, which consists of 3D models across 13 object categories. We use the training, validation and testing splits provided by \cite{3dr2n2} to be comparable to other baselines. We use rendered views from \cite{3dr2n2} and sample 3D points using \cite{shapenetmanifold}.

\begin{figure}[!!t]
  \centering
  \includegraphics[width=\linewidth]{Images/AE/AE.pdf}
%   \captio
\caption{AE results}
\label{AE}
\end{figure}

\vspace{-0.2cm}
\paragraph{Evaluation criteria}
We evaluate the predicted  shape $\mathcal{M}_P$ for geometric accuracy to the ground truth $\mathcal{M}_T$ as well as for manifoldness. For geometric accuracy, we follow \cite{meshrcnn} and compute the bidirectional Chamfer distance according to \eqref{CD} and normal consistency using \eqref{NC} on 10000 points sampled from each mesh. Since Chamfer distance is sensitive to the size of meshes, we scale the meshes to lie within a unit radius sphere. With $\Tilde{M_P},\Tilde{M_T}$ the point sets sampled from $\mathcal{M}_p,\mathcal{M}_T$ and $\Lambda_{P,Q} = \{(p,argmin_{q} ||p-q||) : p \in P\}$, we define
\begin{equation}
    \mathcal{L}_{n} =  |\Tilde{M_P}|^{-1} \!\!\!\! \sum_{(p,q)\in \Lambda_{\Tilde{M}_P,\Tilde{M}_T}} \!\!\!\! |u_p \cdot u_q| \: + \: |\Tilde{M_T}|^{-1} \!\!\!\! \sum_{(p,q)\in \Lambda_{\Tilde{M}_T,\Tilde{M}_P}} \!\!\!\! |u_q \cdot u_p| \: - \: 1
    \label{NC}
\end{equation} 

We detect non-manifold vertices and edges using \cite{open3d} and report the metrics `NM-vertices', `NM-edges' respectively as the ratio of number of non-manifold vertices and edges to total number of vertices and edges in a mesh. To calculate non-manifold faces, we count number of times adjacent face normals have a negative inner product, then the metric `NM-Faces' is reported as its ratio to the number of edges in the mesh. To calculate the number of instances of self-intersection, we use \cite{torch-isect} and report the ratio of number of intersecting triangles to total number of triangles in a mesh.

\vspace{-0.2cm}
\paragraph{Baselines}
We compare with previously published state-of-the-art shape generation methods. This primarily includes direct mesh generation methods Pixel2Mesh \cite{pixel2mesh,meshrcnn}, MeshRCNN  \cite{meshrcnn} and AtlasNet \cite{AtlasNet}. We use pretrained models for all these baselines motioned in this paper since they share the same dataset split by \cite{3dr2n2}. We use the implementation of Pixel2Mesh provided by MeshRCNN, as it uses a deeper network that outperforms the original implementation. We also consider AtlasNet-O which is a baseline proposed in \cite{AtlasNet} that uses patches sampled from a spherical mesh, making it closer to our own choice of initial template mesh. We also create a baseline of our own called NMF-M, which is similar in architecture to NMF but trained with a larger icosphere of 2520 vertices, leading to slight differences in test time performance. To account for possible variation in manifoldness due to simple post processing techniques, we also report outputs of all mesh generation methods with 3 iterations of Laplacian smoothing. Further iterations of smoothing lead to loss of geometric accuracy without any substantial gain in manifoldness. 
We also compare with occupancy networks \cite{OccNet}, a state-of-the-art indirect mesh generation method based on implicit surface representation. Since OccNet is several orders of magnitude slower than direct mesh generation methods, we compare with several variants of OccNet based on the resolution of Multi Iso-Surface Extraction algorithm \cite{OccNet}. For fair comparison to other baselines, we use OccNet's refinement module to output its meshes with 5200 faces.     

\vspace{-0.2cm}
\paragraph{Auto-encoding 3D shapes}
In this section we evaluate NMF's ability to generate a shape given an input 3D point cloud and compare against AtlasNet\cite{AtlasNet} and AtlasNet-O\cite{AtlasNet}.  We evaluate the geometric accuracy and manifoldness of generated meshes. Additionally, we show physically based renderings of generated meshes with dielectric and conductor materials to highlight artifacts due to non-manifoldness. We report the quantitative results for shape generation from point clouds in Table \ref{AE_table}. We report only the weighted mean here and per category results can be found in supplementary material. Notice that NMF outperforms both AtlasNet\cite{AtlasNet} and AtlasNet-O\cite{AtlasNet} in terms of self-intersection with as much as 60 times less instances of self-intersections. Interestingly, even after applying laplacian smoothing, AtlasNet-O\cite{AtlasNet} has 20 times the self-intersections compared to NMF lacking any smoothing. With laplacian smoothing, our method becomes practically intersection free. NMF also outperform the baselines with and without smoothing in terms of non-manifold faces by as much as 1.5 times. Our method generate meshes with a higher normal consistency and therefore they give more realistic results from simulations and physically based rendering applications. It is important to note that AtlasNet\cite{AtlasNet} used 25 mesh templates to construct the final mesh. Since these templates are not closed, the boundary edges are non-manifold (associated to a single face) and hence we get a constant value of 7404 for its non-manifold edges. Both AtlasNet-O and NMF deform a manifold sphere which has manifold edges. All the three methods have manifold vertices.  We show visualizations for two samples in Fig. \ref{AE}. In the first row we notice that AtlasNet\cite{AtlasNet} has severe self-intersections (red) and flipped normals (black) whereas they are minimal for NMF. While the overall geometry of the meshes are similar, these non-manifoldness leads to a big difference in physically based rendering quality. The second row shows meshes with dielectric material. Notice the reflection of red box through chair's backrest is quite realistic for NMF and is close to the ground truth. A harder feature is the green ball besides one of the legs. Notice its reflections is visible through the chair for NMF whereas i is scrambled for AtlasNet-O and completely blocked for AtlasNet. The flipped normals are more problemaitc when it comes to rendering conductor material. Notice the reflections of blue ball onto the chair. NMF is again more realistic and closer to ground truth whereas both variants of AtlasNet struggle with huge black spots in their renderings. 

% \begin{table}
%   \resizebox{\textwidth}{!}{\begin{tabular}{|l|l l l|l l l|l l l|l l l|l l l|l l l|l l l|}
%     \hline
%     \multirow{3}{*}{} &
%       \multicolumn{3}{c|}{Chamfer-L2 ($\downarrow$)} &
%       \multicolumn{3}{c|}{Normal Consistency ($\uparrow$)} &
%       \multicolumn{3}{c|}{NM-Vertices ($\downarrow$)} &
%       \multicolumn{3}{c|}{NM-Edges ($\downarrow$)} &
%       \multicolumn{3}{c|}{NM-Faces ($\downarrow$)} &
%       \multicolumn{3}{c|}{Self-Intersection ($\downarrow$)} \\
%     &AtNet&AtNet-O&NMF&AtNet&AtNet-O&NMF&AtNet&AtNet-O&NMF&AtNet&AtNet-O&NMF&AtNet&AtNet-O&NMF&AtNet&AtNet-O&NMF\\
%     \hline
%     table  & 8.65 & \textbf{4.38} & 7.08 & 0.837 & 0.842 & \textbf{0.853} & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 2.10 & 1.97 & \textbf{1.19} & 28.22 & 9.42 & \textbf{0.20}\\
%     couch  & 2.84 & \textbf{1.98} & 3.24 & 0.679 & 0.668 & \textbf{0.691} & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 1.02 & 0.44 & \textbf{0.14} & 26.96 & 0.80 & \textbf{0.01}\\
%     speak. & \textbf{5.46} & 5.50 & 7.30 & 0.680 & 0.679 & \textbf{0.710} & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 0.40 & 0.14 & \textbf{0.04} & 22.74 & 0.28 & \textbf{0.01}\\
%     firea. & \textbf{1.20} & 1.88 & 2.19 & 0.975 & 0.975 & \textbf{0.977} & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 2.17 & 1.51 & \textbf{0.01} & 24.86 & 6.46 & \textbf{0.00}\\
%     plane  & \textbf{1.11} & 1.20 & 2.76 & 0.938 & 0.939 & \textbf{0.957} & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 2.96 & 2.51 & \textbf{0.91} & 22.75 & 10.07 & \textbf{0.04}\\
%     chair  & \textbf{3.80} & 5.19 & 5.87 & 0.682 & 0.697 & \textbf{0.704} & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 2.01 & 1.89 & \textbf{1.63} & 22.94 & 7.85 & \textbf{0.20}\\
%     monit. & 1.76 & \textbf{1.57} & 2.27 & 0.734 & \textbf{0.737} & 0.699 & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 0.76 & 0.80 & \textbf{0.02} & 25.94 & 2.83 & \textbf{0.00}\\
%     phone  & 1.74 & \textbf{1.40} & 2.36 & \textbf{0.910} & 0.765 & 0.765 & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 0.23 & 0.05 & \textbf{0.02} & 23.98 & 0.16 & \textbf{0.00}\\
%     boat   & \textbf{1.60} & 2.36 & 4.66 & 0.835 & 0.838 & \textbf{0.849} & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 0.86 & 0.47 & \textbf{0.02} & 20.90 & 2.73 & \textbf{0.02}\\
%     lamp   & \textbf{6.21} & 7.00 & 19.24 & 0.917 & \textbf{0.924} & 0.923 & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 1.11 & 2.18 & \textbf{0.82} & 16.8 & 9.01 & \textbf{0.21}\\
%     bench  & 2.13 & \textbf{1.81} & 3.02 & 0.917 & 0.917 & \textbf{0.926} & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 2.41 & 1.65 & \textbf{0.60} & 24.17 & 6.95 & \textbf{0.06}\\
%     car    & 3.00 & \textbf{2.74} & 3.51 & 0.770 & 0.781 & \textbf{0.805} & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 1.37 & 0.49 & \textbf{0.08} & 30.67 & 1.43 & \textbf{0.01}\\
%     cabin  & 3.69 & \textbf{3.53} & 4.10 & \textbf{0.900} & 0.897 & 0.896 & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 0.67 & 0.23 & \textbf{0.15} & 26.64 & 0.62 & \textbf{0.01}\\
%     \hline
%     mean   & 4.15 & \textbf{3.50} & 5.54 & 0.815 & 0.816 & \textbf{0.826} & 0.00 & 0.00 & 0.00 & 7.40 & \textbf{0.00} & \textbf{0.00} & 1.72 & 1.43 & \textbf{0.71} & 24.80 & 6.03 & \textbf{0.10}\\
%     mean (with Laplace)   & 4.59 & 3.81 & 5.25 & 0.807 & 0.811 & \textbf{0.826} & 0.00 & 0.00 & 0.00 & 7.40 & 0.00 & 0.00 & 0.47 & 0.56 &0.38 & 13.26 & 2.02 & \textbf{0.00}\\
%     \hline
    
%   \end{tabular}}
%   \caption{Auto Encoding Performance}
% \end{table}
\begin{table}
  \resizebox{\textwidth}{!}{\begin{tabular}{|l|l l l|l l l|l l l|l l l|l l l|}
    \hline
    \multirow{3}{*}{} &
      \multicolumn{3}{c|}{Chamfer-L2 ($\downarrow$)} &
      \multicolumn{3}{c|}{Normal Consistency ($\uparrow$)} &
    %   \multicolumn{3}{c|}{NM-Vertices ($\downarrow$)} &
    %   \multicolumn{3}{c|}{NM-Edges ($\downarrow$)} &
      \multicolumn{3}{c|}{NM-Faces ($\downarrow$)} &
      \multicolumn{3}{c|}{Self-Intersection ($\downarrow$)} \\
    &AtNet&AtNet-O&NMF&AtNet&AtNet-O&NMF&AtNet&AtNet-O&NMF&AtNet&AtNet-O&NMF\\
    \hline
    mean   & 4.15 & \textbf{3.50} & 5.54 & 0.815 & 0.816 & \textbf{0.826} & 1.72 & 1.43 & \textbf{0.71} & 24.80 & 6.03 & \textbf{0.10}\\
    mean (with Laplace)   & 4.59 & \textbf{3.81} & 5.25 & 0.807 & 0.811 & \textbf{0.826} & 0.47 & 0.56 &\textbf{0.38} & 13.26 & 2.02 & \textbf{0.00}\\
    \hline
    
  \end{tabular}}
  \caption{Auto Encoding Performance}
  \label{AE_table}
\end{table}



\vspace{-0.2cm}
\paragraph{Single-view reconstruction}

\begin{table}
  \resizebox{\textwidth}{!}{\begin{tabular}{|l|l l|l l|l l|l l|l l|l l|l l|}
    \hline
    \multirow{2}{*}{} &
      \multicolumn{2}{c|}{Chamfer-L2 ($\downarrow$)} &
      \multicolumn{2}{c|}{Normal Consistency ($\uparrow$)} &
      \multicolumn{2}{c|}{NM-Vertices ($\downarrow$)} &
      \multicolumn{2}{c|}{NM-Edges ($\downarrow$)} &
      \multicolumn{2}{c|}{NM-Faces ($\downarrow$)} &
      \multicolumn{2}{c|}{Self-Intersection ($\downarrow$)} \\
   &  & w/ Laplace & & w/ Laplace & & w/ Laplace & & w/ Laplace & & w/ Laplace & & w/ Laplace\\
    \hline
   MeshRCNN\cite{meshrcnn}       & \textbf{4.73} & \textbf{5.96} & 0.698 & 0.758 & 9.32 & 9.32 & 17.88 & 17.88 & 5.18 & 0.86 & 7.07 & 1.41 \\
   Pixel2Mesh\cite{pixel2mesh}   & 5.48 & 10.79 & 0.706 & 0.720 & 0.00 & 0.00 & 0.00 & 0.00 & 3.33 & 0.88 & 12.29 &  6.52 \\ 
   AtlasNet-25\cite{AtlasNet}    & 5.48 & 7.76 & 0.826 & 0.824 & 0.00 & 0.00 & 7.40 & 7.40 & 1.76 & 0.48 &26.94 & 17.57 \\
   AtlasNet-sph\cite{AtlasNet}   & 6.67 & 7.35 & 0.838 & 0.836 & 0.00 & 0.00 & 0.00 & 0.00 & 2.19 & 1.08 & 11.07 &5.94 \\
\hline
  NMF                            & 7.82 & 8.64 & 0.829 & 0.837 & 0.00 & 0.00 & 0.00 & 0.00 & 0.83 & 0.45 & 0.12 &\textbf{0.00} \\
  NMF-M                          & 9.05 & 8.73 & \textbf{0.839} & \textbf{0.838} & \textbf{0.00} & \textbf{0.00} & 0.00 & 0.00 & \textbf{0.76} & \textbf{0.42} & \textbf{0.11} & \textbf{0.00}\\
    \hline
    
  \end{tabular}}
  \caption{Single View Reconstruction}
  \label{SVR_table}
\end{table}

We evaluate the potential of our method for single-view reconstruction and compare against state-of-the-art methods AtlasNet\cite{AtlasNet}, AtlasNet-O\cite{AtlasNet}, Pixel2Mesh\cite{meshrcnn,pixel2mesh} and MeshRCNN\cite{meshrcnn}. The quantitative results are reported in Table \ref{SVR_table} where we only show the mean of various metrics over shapenet categories. We notice that self-intersections in NMF are significantly lower (about 60 times) than best baseline and are practically zero with laplace smoothing. Whereas with the possible exception of MeshRCNN\cite{meshrcnn} all other baselines suffer from severe self-intersections even after laplace smoothing. Our method again results in fewer than 50\% non-manifold faces compared to the best baseline. NMF-M also gets the highest normal consistency performance. Due to the \textit{cubify} step as part of the MeshRCNN\cite{meshrcnn} pipeline which converts a voxel grid into mesh, the method has several non-manifold vertices and edges compared to deformation based methods Pixel2Mesh\cite{pixel2mesh}, AtlasNet-O\cite{AtlasNet} and NMF. AtlasNet\cite{AtlasNet} suffers from the most number of non manifold edges almost 100 times that of MeshRCNN\cite{meshrcnn}. We observe that while being poor in terms of manifoldness, MeshRCNN\cite{meshrcnn} outperforms other baselines in terms of chamfer distance. We qualitatively show the effects of non-manifoldness in Fig. \ref{SVR_table}-\ref{SVR_chair}. We observe that for dielectric material (second row) NMF is able to pass on the background colors closest to that of the ground truth whereas other baselines only reflect the white sky due to the presence of flipped normals. 

\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{Images/SVR/SVR-table.pdf}
%   \captio
\caption{SVR results}
\label{SVR_table}
\end{figure}

\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{Images/SVR/SVR-chair.pdf}
%   \captio
\caption{SVR results}
\label{SVR_chair}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{Images/SVR/Occnet2.pdf}
%   \captio
\caption{Comparison with Implicit methods}
\label{fig:fig}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{Images/ablation.pdf}
%   \captio
\caption{Ablation}
\label{fig:fig}
\end{figure}


==> _OLD_intro.tex <==

\section{Introduction}
Mesh representation for 3D objects are a promising approach for encoding the structure of 3D objects. They provide a cheap and efficient virtual representation of physical entities and are widely used in computer graphics, modelling, simulation and additive manufacturing etc. In order to get desirable results, the mesh representations, in addition to being geometrically accurate, are required to be \textit{manifold}. This prevents ambiguities while using techniques like ray tracing, slicing and mesh boolean operations resulting in physically consistent results (see Fig. \ref{teaser}). A manifold is defined as a topological space that locally resembles Euclidean space in the neighbourhood of each point. A manifold mesh is a discretization of the manifold using a disjoint set of simple 2D polygons like triangles. Such a discretization is simpler to work with when designing simulations, rendering and other manifold calculations. While a mesh data structure can simply be defined as a set $(\mathcal{V},\mathcal{E}, \mathcal{F})$ of vertices $\mathcal{V}$ and corresponding edges $\mathcal{E}$ or face $\mathcal{F}$, not every mesh $(\mathcal{V},\mathcal{E}, \mathcal{F})$ is manifold. Intuitively, a mesh exhibit manifold property only when it can be realized physically (say by 3D printing). Mathematically, we list various constraints on a singly connected mesh with the set $(\mathcal{V},\mathcal{E}, \mathcal{F})$ that enables \textit{manifoldness}. 

\begin{figure}
    \centering
    \includegraphics[width=0.25\linewidth]{Images/manifoldness.pdf}
    \caption{Non-manifold geometries for a part of singly connected mesh: (a) An edge that is shared by either exactly one (red) or more than two (red dashed) faces. (b) A vertex (red) shared by more than one group of connected faces. (c) Adjacent faces that have normals (red-arrow) oriented in opposite directions. (d) faces intersecting other triangles of the same mesh.  }
    \label{manifoldness}
\end{figure}

\begin{itemize}
    \item Edge $e\in\mathcal{E}$ is common to exactly 2 faces in $\mathcal{F}$ (Fig \ref{manifoldness} a)
    \item Vertex $v\in\mathcal{V}$ shared by exactly one group of connected faces (Fig \ref{manifoldness} b)
    \item Adjacent faces $F_i, F_j$ have normals oriented in same direction (Fig \ref{manifoldness} c)
    % \item Each element occurs only once in the set $(\mathcal{V},\mathcal{E}, \mathcal{F})$
\end{itemize}{}
The above mentioned constraints on a mesh $(\mathcal{V},\mathcal{E}, \mathcal{F})$ guarantees to be a manifold in the limit that the manifold discretization is infinitesimally small. This is not the case when dealing with practical meshes that often have large areas and are non-uniformly spread. Such meshes often have \textit{self-intersections} (Fig \ref{manifoldness} d) which occur when two or more triangles belonging to the same mesh intersect one another. It is easy to observe that a mesh with manifold vertices, edges and faces
can have \textit{self-intersections} failing it to be realized physically. In the scope of this work, we therefore tighten the definition of manifold meshes to exclude those meshes that have \textit{self-intersections} to arrive at a more useful definition for practical meshes. 

\begin{figure}[t]
\centering
\begin{minipage}{0.1\textwidth}
\centering
 \includegraphics[width=\linewidth]{Images/Teaser/inputs.pdf}
 \vspace{-0.2in}
 \subcaption{Possible Inputs}
 \label{fig:env_atk}
\end{minipage}\quad
\begin{minipage}{0.3\linewidth}
	\label{manifoldness_overview}
	\centering
	\resizebox{\textwidth}{!}{\begin{tabular}{llllll}
\toprule
% \multicolumn{2}{c}{Part}                   \\
\cmidrule(r){1-2}
    & Approach & Vertex  & Edge & Face & Non-Int. \\
\midrule
MeshRCNN\cite{meshrcnn} & explicit & \xmark  & \xmark & \xmark & \xmark     \\
AtlasNet\cite{AtlasNet} & explicit & \cmark  & \xmark & \xmark & \xmark     \\
AtlasNet-O\cite{AtlasNet} & explicit & \cmark  & \cmark & \xmark & \xmark     \\
Pixel2Mesh\cite{pixel2mesh} & explicit & \cmark  & \cmark & \xmark & \xmark     \\
GEOMetrics\cite{geometrics} & explicit & \cmark  & \cmark & \xmark & \xmark     \\
3D-R2N2\cite{3dr2n2} & implicit & \xmark  & \xmark & \cmark & \cmark     \\
PSG\cite{PSG} & implicit & \xmark  & \xmark & \cmark & \cmark     \\
OccNet\cite{occupancy} & implicit & \xmark  & \xmark & \cmark & \cmark     \\
\cmidrule(r){1-6}
\textbf{NMF (Ours)}& explicit & \textbf{\cmark}  & \textbf{\cmark} & \textbf{\cmark} & \textbf{\cmark}     \\
\bottomrule
\end{tabular}}
	\subcaption{Manifoldness of prior work}
\end{minipage}\quad
\begin{minipage}{0.4\textwidth}
\centering
 \includegraphics[width=\linewidth]{Images/Teaser/appliations_enabled.pdf}
 \vspace{-0.2in}
 \subcaption{Applications enabled by NMF Manifold Meshes}
 \label{teaser}
\end{minipage}
\caption{Given an input as either a 2D image or a 3D point cloud (a) Existing methods generate corresponding 3D mesh that fail one or more manifoldness conditions (b) yielding unsatisfactory results for various applications including physically based rendering (c). NeuralMeshFlow generates manifold meshes which can directly be used for high resolution rendering, physics simulations (see supplementary video) and be 3D printed without the need for any prepossessing or repair effort.}
\end{figure}

% \begin{figure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/toy/circle.pdf}
%   \caption{Spherical mesh}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/toy/star.pdf}
%   \caption{Star mesh}
%   \label{fig:sfig2}
%   \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/toy/star-mlp.pdf}
%   \caption{Only Chamfer Distance}
%   \label{fig:sfig2}
% \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/toy/star-edge.pdf}
%   \caption{With Edge Length regularization}
%   \label{fig:sfig2}
%   \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/toy/star-lap.pdf}
%   \caption{with Edge Length and Laplacian regularization}
%   \label{fig:sfig2}
%   \end{subfigure}
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{Images/toy/star-nmf.pdf}
%   \caption{Bu using a NeuralODE}
%   \label{fig:sfig2}
%   \end{subfigure}
% \caption{2D Toy example}
% \label{toy}
% \end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Images/toy.pdf}
    \caption{2D Toy Example: For the task of deforming a manifold template mesh (a) to a target mesh (b) using explicit mesh regularization (c-e) trades edge-intersections for geometric accuracy . In contrast, a NODE\cite{NODE} (f) is implicitly regularized preventing edge-intersections without loosing geometric accuracy.}
    \label{toy}
\end{figure}

Existing learning based surface generation methods, while giving impressive geometric accuracy, fail one or more \textit{manifoldness} conditions (Fig. \ref{teaser} b). While the indirect approaches \cite{3dr2n2,PSG,OccNet,deepsdf,DeepLevelSets,ImplicitFields} fail because of the non-manifoldness of marching cube algorithm \cite{marching} (refer section 2 for details), direct methods \cite{meshcnn}\cite{pixel2mesh}\cite{AtlasNet}\cite{geometrics} suffer from what we call the \textit{regularizer's dilemma}. The dilemma refers to the trade-off between geometric accuracy and higher manifoldness. We explain this dilemma with the help of a 2D toy example (Fig. \ref{toy}). Consider the task of deforming a template unit spherical mesh $S$ (Fig \ref{toy} (a)) into a target star mesh $T$ (Fig. \ref{toy} b). Let's use a multi layer perceptron $f_{\theta}$ with a unit hidden layer of $256$ neurons with $relu$ and output layer with $tanh$ activation to approximate this deformation. We can train $f_{\theta}$ by minimizing some loss $L$ over the points sampled from $S, T$. A naive approach involves minimizing the Chamfer Distance $L_c$ between $S, T$ which leads to accurate point predictions but has several edge-intersections (Fig. \ref{toy}c). By introducing edge length regularization $L_e$ we get fewer edge-intersections (Fig \ref{toy}d) but the solution is also sub-optimal geometrically. We can further bring down the edge-intersections by including Laplacian regularization (Fig \ref{toy}e) however this takes a bigger toll on geometric accuracy. This demonstrates that an attempt to reduce self-intersections by introducing explicit regularization terms not only makes the optimization hard but often lead to unpleasant predictions with lower geometric accuracy. In this work, we hypothesize that NODE\cite{NODE} (with dynamics $f_{\theta}$) are implicitly regularized by construction to prevent self-intersections \cite{NODEapprox}\cite{ANODE} and thus do not require any explicit regularization which let's us resolve the dilemma.  

In this work we exploit the property of NODE\cite{NODE} of being implicit regularizers against self-intersections to do 3D manifold mesh generation. Our proposed model NeuralMeshFlow consists of several NODE blocks that successively learn to deform a spherical template mesh to a target given its encoding.
% We explain this dilemma with the help of a 2D toy example (Fig. \ref{toy}). Consider the task of deforming a template unit spherical mesh $S$ (Fig \ref{toy} (a)) into a target star mesh $T$ (circumscribed by $S$, see Fig. \ref{toy} b). We wish to fit a function $f_{\theta}:S\subset\mathbb{R}^2 \rightarrow \mathbb{R}^2$ parameterized by $\theta$ that predicts the deformed position $\hat{y} = f_{\theta}(x)$ for every point $x\in S$. Here we take a multi layer perceptron with a unit hidden layer of $256$ neurons with $relu$ and output layer with $tanh$ activation. For simplicity, we will uniformly sample $N=60$ points from both $S,T$ to get the point sets $\Tilde{S},\Tilde{T}$. We can get the desired mapping by solving the optimization problem $\theta^* = arg\min_{\theta} L(\Tilde{S},\Tilde{T})$ for some loss $L$. A naive approach of only minimizing the Chamfer Distance $L_c$ between $\Tilde{S},\Tilde{T}$ leads to accurate point predictions but is filled with edge self-intersections (Fig. \ref{toy}c). By introducing edge length regularization $L_e$ we get fewer self-intersections (Fig \ref{toy}d) but the solution is also sub-optimal. We can further bring down the edge-intersections by including Laplacian regularization (Fig \ref{toy}e) however this leads to inferior geometric accuracy. This demonstrates that an attempt to reduce self-intersections by introducing explicit regularization terms not only makes the optimization hard but often lead to unpleasant predictions with lower geometric  accuracy. 

% For starters, we let $L=L_c$, where $L_c$ is the Chamfer Distance between $\Tilde{S},\Tilde{T}$. Solving this optimization we get result shown in Fig. \ref{toy}(c). As we can observe, the mapping can accurately overlay points $x\in\Tilde{S}$ on $\Tilde{T}$ minimizing $L$ but the edges are intersecting at several locations causing an otherwise manifold spherical template to be deformed into a non-manifold geometry. One way to handle this would be introduce some edge length regularizing term in $L = \lambda_1 L_c + \lambda_2 L_e$, where $L_e$ penalizes edges longer edges. While this approach leads to fewer self-intersections (Fig \ref{toy}d), it doesn't stop it altogether. We can increase the regularization even more by adding some Laplacian regularization $L = \lambda_1 L_c + \lambda_2 L_e + \lambda_3 L_l$ where $L_l$ penalizes sharp changes of laplacian coordinates before and after the deformation which leads
% Meshes provide a natural way of representing 3D entities in terms of their boundary information. This is because these virtual entities interact with each other and their surroundings based on the information contained in their boundaries. This is why for applications like physics simulation, physically based rendering, etc, it is important to know correct mesh boundaries. This fact is so critical to the functioning of these applications that all other 3D representations are first converted into meshes to enable any of these. It is therefore important to describe what is a \textit{correct} mesh. In this work, we make the key insight that a \textit{correct} mesh ought to interact with the virtual world like the real object it represents. Applications like physically based rendering, simulation and 3D printing frequently require meshes to be \textit{manifold}.  
% A mesh based representation of 3D shapes has several advantages over other representations namely point clouds, SDF, voxels, etc. Compared to SDFs and voxel based representations, meshes are cheaper to store and process while still retaining the valuable connectivity information which is not present in point clouds. The reason behind such efficiency gains is the underlying assumption that these virtual objects interact with their surroundings as mere surfaces. This straightaway gives an order of n memory savings when working in 3D, this means a lot. Treating objects as surface is not only beneficial from a memory and computation point of view but is infact critical for applications like ray tracing and physics simulations since given a surface it is trivial to find out wheter a point is inside or outside the ssurface. 

% Recently, significant progress has been made on learning good representations for 3D point clouds\cite{pointflow}\cite{foldingnet}\cite{PSG}, SDFs\cite{deepsdf}\cite{occupancy} and voxels\cite{3dr2n2}. However, learning a representations for generating high-resolution 3D meshes still remains an open challenge due to several reasons. Firstly, designing convolution operators on meshes is far from trivial \cite{meshcnn}\cite{scan2mesh}. Unlike voxels and point clouds, there is not a well defined concept of `neighbourhood' which is critical to the functioning of deeper networks. One way to circumvent these challenges is to do mesh generation by predicting point clouds instead and imposing shape regularizations to ensure that underlying topology is appropriate \cite{AtlasNet}. However, this approach assumes that better point cloud predictions \textit{ipso facto} implies better mesh prediction. This is not true as better mesh predictions require accurate surface normal, laplacians, etc in addition to point locations. Moreover, employing shape regularizers is not insufficient to generate manifold meshes but also lead to optimization difficulties  which lead to limited applicability of such methods in real life use. 

In summary, we make the following contributions to 3D mesh generation research.

\begin{itemize}
    \item We propose a novel approach to 3D mesh generation with NeuralMeshFlow (NMF), which is made up of a series of NODE blocks that learn to deform a template mesh (ellipsoid) into the target shape that encourages \textit{manifoldness} of generated mesh.

    \item We carry out extensive evaluations of state-of-the-art mesh generation methods for physically based rendering and simulation (see supplementary video) to highlight that they fail to give realistic results due to absence of manifoldness.
    % \item Through extensive evaluation, we highlight that contemporary methods while good at predicting the geometry of meshes fail to generate manifold meshes and limit their applicability in real life. 
    \item We also show applications to single-view reconstruction, 3D deformation, global parameterization and correspondence capabilities of NMF.
    
\end{itemize}{}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Images/Teaser/teaser-crop.pdf}
%     \caption{Given an input 2D image or a 3D point cloud (a), the corresponding 3D meshes generated from NeuralMeshFlow are \textit{manifold} that enable applications like Physics Simulation (b) 3D printing (c) and Physically based rendering for complex materials such as dielectrics (d left) which is not possible from other state-of-the-art mesh generation methods (d right) due to non-manifold geometry}
%     \label{fig:my_label}
% \end{figure}

% \section{Background}
% We begin with an overview of manifold meshes and define various terminologies used in this work. We then provide a brief overview of Neural Ordinary Differential Equations (NODE) and cover some of the relevant properties regarding Homeomorphism and Flows. 

% \subsection{Manifold Mesh}

% In three dimensions, this means that given a manifold $\mathcal{X}\subset\mathbb{R}^3$ very point $p\in\mathcal{X}$ will have an open set $\mathcal{W}\subset\mathcal{X}$ containing p which is homeomorphic to 

% \subsection{Neural ODE}




% Neural ODEs are proposed as a generalization to the deep residual networks [add citations]. In a typical residual block, the difference between the output and input is modelled by a neural network $f_{\Theta}: \mathbb{R}^n \rightarrow \mathbb{R}^n$ which is parameterized by $\Theta$. Intuitively, this means that an input $x_0 \in \mathbb{R}^n$ is subsequently evolved as $x_t$ in discrete time steps $t \in \{1,2,..,N\}$ by the $N$ hidden layers  (eq. \ref{residual}). 

% \begin{equation}
%     x_{t+1} - x_{t} = f_{\Theta}(x_t)
%     \label{residual}
% \end{equation}

% This dynamics can be seen as an Euler approximation to the first order differential equation (eq. \ref{firstorderdiff}) where in the limit as $h_t \rightarrow 0$ the discrete hidden layers converge to form a `continuum' of shared parameters for the entire network and the input $x_0$ is said to \textit{flow} in time $t \in \mathbb{R}$. 

% \begin{equation}
%     \frac{dx_t}{dt} = \lim_{h_t \rightarrow 0} \frac{x_{t+h_t} - x_t}{h_t} = f_{\Theta}(x_t)
%     \label{firstorderdiff}
% \end{equation}{}

% Thus instead of learning the transformation $\phi_T: \mathcal{X} \rightarrow \mathcal{X}$ by a finite layer deep neural network, a Neural ODE learns it indirectly, through the solutions to the initial value problem (IVP) of the ODE (eq. \ref{ODEeq}). Here $x_0, x_T \in \mathcal{X} \subset \mathbb{R}^n$ represent the input and output from the network respectively, while $T\in \mathbb{R}$ is a hyper parameter which represents the duration of the \textit{flow} from $x_0$ to $x_T$.
% \begin{equation}
%     x_T = \phi_T(x_0) = x_0 + \int_0^T f_{\Theta}(x_t)dt
%     \label{ODEeq}
% \end{equation}{}

% The adjoint sensitivity \cite{adjointsensitivity} method is often employed to perform the reverse-mode differentiation through the ODE solver and therefore learn the network parameters $\Theta$ using the standard gradient descent approaches. 

% The NODE formulation has several benefits including better parameter efficiency, modelling of continuous time dynamics, invertibility and easy calculation of normalizing flows. In this work we exploit the fact that NODE are capable of learning a restricted set of \textit{homeomorphism} \cite{NODEapprox}. By observing the definition of NODE (see eq. \ref{ODEeq}) we see that $\phi_T:\mathcal{X}\rightarrow\mathcal{X}$ is continuous, bijective and its inverse $\phi_T^{-1} = \phi_{-T}$ exists and is also continuous. Therefore it is safe to say that any NODE with a well behaved dynamics $f_{\Theta}$ (Lipschitz continuous) learns a homeomorphism on $\mathcal{X}$. The property of \textit{homeomorphism} is central to dealing with manifolds as it allows for converting one manifold into another without destroying the underlying topology. 

% However, as pointed out by \cite{NODEapprox}, NODE cannot learn homeomorphic mappings that requires distinct trajectories to intersect. It is easy to show by training to fit NODE on a simple 1-D problem $g(x)=-x \ , x\in \mathbb{R}$. The NODE of any complexity will fail to fit the function $g(x)$ as this would involve intersecting the trajectories $x_0=-1 \rightarrow x_T=1$ and $x_0=1 \rightarrow x_T=-1$. The reason behind this is that if two distinct trajectories indeed intersected at $x_*$ for some $t=t^*$ then solving $\phi_{-t^*}(x^*)$ would always give a unique value which would result in a contradiction. The fact that NODE implicitly discourage trajectories that self-intersect allows for learning smooth non-intersecting \textit{homeomorphic deformation} of a manifold $\mathcal{X}\rightarrow\mathcal{Y}$.

%  Given a topological space $\mathcal{X} \in \mathbb{R}^n$, a mapping $h: \mathcal{X} \rightarrow \mathcal{X}$ is said to be a \textit{homeomorphism} if $h$ is bijective whose inverse exists and is continuous. 
% learning  \textit{topological transformation group} or \textit{flow} \cite{NODEapprox} which allows . 
% can a restricted set of homeomorphism.
%  Surprisingly, . 
 

% \begin{itemize}
%     \item Need to mention the related work on NODEs?
% \end{itemize}{}



==> _OLD_method.tex <==
% \section{NeuralMeshFlow}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{Images/pipeline.pdf}
%   \captio
\caption{NeuralMeshFlow consists of three deformation blocks that perform subsequent point-wise flow on spherical mesh vertices based on the shape embedding $z$ from target shape $\mathcal{M}_T$. The bottom row shows an actual chair being generated at various instants of NMF. Time instances $0<T_1<T_2<T$ show the deformation of spherical mesh into a coarse chair representation $\mathcal{M}_{p0}$ by first deformation block. Further deformation blocks perform subsequent refinements to get $\mathcal{M}_{p1}, \mathcal{M}_{p2}$.}
\label{pipeline}
\end{figure}

\section{NeuralMeshFlow}

In this section we introduce NeuralMeshFlow (Fig \ref{pipeline}), which learns to auto-encode 3D shapes. Given a 3D shape, $M_T$, we uniformly sample $N=2520$ points from its surface and feed to a PointNet\cite{pointnet} encoder which gives us the shape embedding $z$ of length $k=1000$. The vertices of an icosphere $M_S$ are passed through six NODE blocks (conditioned on $z$) across the three deformation blocks yielding vertices of the predicted shape. Since NMF does not alter the mesh topology, we simply use the connectivity information of icosphere to generate shapes $M_{p1}, M_{p2}$ from respective predicted vertices. In this section, we first briefly discuss the implicit shape regularization in NODE. We then explain the dynamics equation $f_{\theta|z}$ which forms the core representation learning part of Neural ODEs. We then describe the deformation flow $F_{\theta|z}$ that does mesh prediction which is then later refined by subsequent flows. Lastly, we discuss about the loss functions used for training NeuralMeshFlow. 

% In this section we introduce our model NeuralMeshFlow, which generates a 3D shape given its encoding. The encoding can either come from a shape or its image. To encode the shape, we uniformly sample 2048 points and feed to a PointNet\cite{pointnet} encoder which gives us the shape embedding $z$ of length $k=1000$. For an image input, a pretrained resnet-18\cite{resnet} encoder is used. We use Neural ODE blocks to learn the deformation flow from initial ellipsoid mesh to target shape. In this section, we first explain the dynamics equation $f_{\theta|z}$ which forms the core representation learning part of Neural ODEs. We then describe the deformation flow $F_{\theta|z}$ that does mesh prediction which is then later refined by subsequent flows. Lastly, we discuss about the loss functions used for training NeuralMeshFlow.
 
 
\paragraph{NODE Overview.} A NODE learns a transformation $\phi_T: \mathcal{X} \rightarrow \mathcal{X}$ as solutions for initial value problem (IVP) of a parameterized ODE (eq.\ref{ODEeq}). Here $x_0, x_T \in \mathcal{X} \subset \mathbb{R}^n$ represent the input and output from the network respectively, while $T\in \mathbb{R}$ is a hyper parameter which represents the duration of the \textit{flow} from $x_0$ to $x_T$. For a well behaved dynamics $f_{\Theta}$ (Lipschitz continuous) the IVP enforces the existence and uniqueness of solutions \cite{ANODE}\cite{NODEapprox} which implies that any two distinct trajectories of NODE can never intersect. The uniqueness property presents several advantages to NODE compared to traditional MLPs such as improved robustness \cite{robustnode}, parameter efficiency \cite{NODE} and the ability to learn normalizing flows \cite{ffjord}\cite{pointflow}\cite{occflow} and homeomorphism \cite{NODEapprox}. As illustrated by the toy example in figure \ref{toy} we argue that regularization against self-intersection non-manifold faces is yet another consequence of the uniqueness and orientation preserving property of NODE. We refer readers to \cite{ANODE}\cite{NODEapprox}\cite{dissectingNODE} for more details. 

\begin{equation}
    x_T = \phi_T(x_0) = x_0 + \int_0^T f_{\Theta}(x_t)dt
    \label{ODEeq}
\end{equation}{}

% \subsection{}
\paragraph{Dynamics Equation.}
The Neural ODE $F_{\theta|z}$  is built around the dynamics equation $f_{\theta|z}$ which is learned by a deep network. Given a point $x\in \mathbb{R}^3$ we first get 512 length point features by applying a linear layer. Then we extract a 512 length shape feature from the shape embedding $z$ and multiply it element wise with the obtained point features to get the \textit{point-shape} features. Lastly, we feed the \textit{point-shape} features into two residual MLP blocks each of width 512 and subsequent MLP of width 512 which outputs the predicted point location $y\in\mathbb{R}^3$. Based on the findings of \cite{identityresnet}\cite{dissectingNODE} we make use of the $tanh$ activation after adding the residual predictions at each step. This ensures maximum flexibility in the dynamics learned by the deep network. 
% Also note that the discussion in section 2.2 can be extended for NMF because the same conditional dynamics is applied to all points belonging to the same object instance. 

\paragraph{Deformation Flow.}
The objective of deformation flow is to learn a conditional mapping $F_{\Theta|z}: \mathcal{M}_I \rightarrow \mathcal{M}_O \subset \mathbb{R}^3$ given the shape embedding $z$. Here $\mathcal{M}_I, \mathcal{M}_O$ refer to the set of input and output points respectively. 

% Instead of working directly with mesh data, we apply deformation flow on the vertices $\mathcal{V}_o$ of the ellipsoidal mesh $\mathcal{M}_o$ to get the vertices $\mathcal{V}_p$ corresponding to the predicted mesh $\mathcal{M}_p$.

\begin{equation}
    p^i_O = F_{\Theta|z}(p^i_I,z)  = p^i_I + \int_0^T f_{\Theta|z}(p^i_I,z)dt
    \label{forward}
\end{equation}{}


For each point $p^i_I\in \mathcal{M}_I$ we solve the \textit{forward flow} (Eq. \ref{forward}) to get the updated point location $p^i_O\in\mathbb{R}^3$ of the output points set. It should be noted that the IVP in eq.\ref{forward} is similar to eq. \ref{ODEeq} in the sense that it also enforces point trajectories $p^i_I \rightarrow p^i_O$ to never intersect. However, here we condition the flow on the shape embedding which allows for different IVPs to be learned for different shapes. We also give the network flexibility to stretch the predicted point cloud along the three axis by means of an instance normalization layer. This is achieved by an MLP with one hidden layer of size 256 that regresses the three scaling factors from the shape embedding $z$.

\paragraph{Refinement Flows.}
We successively apply the deformation flow in Eq. \ref{forward} to get two additional refinement flows. Therefore, the entire NMF can be seen as three successive deformation flows $\{F^0_{\Theta|z},F^1_{\Theta|z},F^2_{\Theta|z}\}$ of the initial ellipsoid to get to the final prediction.

% Once we have the set of predicted vertices $\mathcal{V}_p = {v^i_p}$, in order to calculate the mesh loss, we create yet another \textit{points}-set which consists of points (and respective point-normals) sampled differentiably \cite{pytorch3d} from the predicted mesh. 
% \paragraph{Instance Normalization :}
% Since we plan to deform a spherical mesh with zero covariance into a target shape with non-zero covariance, it would require some set of points to be \textit{flowed} by a larger amount than others. But we keep the time duration of integration for the entire deformation flow constant for all the points, to get implicit shape regularization. This therefore leads to more complex dynamics being learned. We avoid this situation by introducing instance normalization layer before and after each deformation flow. 
\paragraph{Loss Function.}
In order to learn the parameters $\Theta$ it is important to use a loss which meaningfully represents the difference between the predicted $M_P$ and the target $M_T$ meshes. To this end we use the bidirectional Chamfer Distance (eq.\ref{CD}) on the points sampled differentiably\cite{pytorch3d} from predicted $\Tilde{M}_P$ and target $\Tilde{M}_T$ meshes.

\begin{equation}
    \mathcal{L}(\Theta) = \sum_{p\in \Tilde{M}_P} \min_{q \in \Tilde{M}_T} || p - q ||^2 +  \sum_{q\in \Tilde{M}_T} \min_{p \in \Tilde{M}_P} || p - q ||^2 
    \label{CD}
\end{equation}

We compute chamfer distances $\mathcal{L}_{p1}, \mathcal{L}_{p2}$ for meshes after deformation blocks $F^1_{\Theta|z}$ and $F^2_{\Theta|z}$. For meshes generated from $F^0_{\Theta|z}$ we found that computing chamfer distance $\mathcal{L}_{v}$ on the vertices gave better results since it encourages predicted vertices to be more uniformly distributed (like points sampled from target mesh). We thus arrive at the overall loss function to train NMF.
\begin{equation}
    \mathcal{L} = w_0\mathcal{L}_v + w_1\mathcal{L}_{p1} + w_2\mathcal{L}_{p2}
\end{equation}
Here we take $w_0 = 0.1, w_1=0.2, w_3=0.7$ so as to enhance mesh prediction after each deformation flow. The adjoint sensitivity \cite{adjointsensitivity} method is employed to perform the reverse-mode differentiation through the ODE solver and therefore learn the network parameters $\Theta$ using the standard gradient descent approaches.

% The monotonic increase in weight values with successive deformations is to have each flow refine its input mesh and not cause competition with each other which leads to inferior results.
% In order to learn the parameters $\Theta$ it is important to use a loss which meaningfully represents the difference between the predicted and the target meshes. However, instead of working directly with mesh data, we form five point-based sets. The first three sets are \textit{vertex}-sets which consists of vertices (and respective vertex-normals) belonging to ellipsoid $(\mathcal{V}_o,\mathcal{N}_{vo})$, target mesh $(\mathcal{V}_t, \mathcal{N}_{vt})$ and target mesh $(\mathcal{V}_p, \mathcal{N}_{vp})$. We then create two \textit{points}-set which consists of points (and respective point-normals) sampled differentiably \cite{pytorch3d} from the target mesh $(\mathcal{P}_t,\mathcal{N}_{pt})$ and predicted mesh $(\mathcal{P}_p,\mathcal{N}_{pp})$.
% For this, we use the well known bidirectional Chamfer Distance.

% \begin{equation}
% \mathcal{L}_f(\Theta) = \sum_{p\in X_0} \min_{q \in X_1} ||\mathcal{F}_{\Theta| z}(p) - q||^2  + \sum_{q\in X_1} \min_{p \in X_2} ||\mathcal{F}_{\Theta| z}(q) - p||^2  
% \end{equation}{}

% However, since NODE has out-of-box invertibility, we make use of it to impose cycle-consistency between $X_0 \xrightarrow{\mathcal{F}_{\Theta| z}} X_1 \xrightarrow{\mathcal{F}_{\Theta| z}^{-1}} X_0$ which we show during the ablation studies gives substantial improvement in performance.


==> _OLD_related.tex <==
\section{Related Work}
\label{sec:related}

Existing learning based mesh generation methods, while yielding impressive geometric accuracy, do not satisfy one or more \textit{manifoldness} conditions (Fig.~\ref{teaser}b). While indirect approaches \cite{3dr2n2,PSG,OccNet,deepsdf,DeepLevelSets,ImplicitFields} suffer from the non-manifoldness of the marching cube algorithm \cite{marching}, direct methods \cite{meshcnn,pixel2mesh,AtlasNet,geometrics} are faced with the \textit{regularizer's dilemma} on the trade-off between geometric accuracy and higher manifoldness, illustrated in Fig.~\ref{toy} and discussed in Sec.~\ref{sec:intro}. 

% Taken from related work of OccNet
% Existing works on 3D mesh generation either directly regress the mesh or indirectly attempt to generate it during post-processing of a voxel, point cloud or implicit function based representation. The indirect approaches differ in the manner in which they predict the surface but use a common iso-surface extraction algorithm which is often some derivative of the Marching Cube algorithm\cite{marching}. Both the direct and indirect approaches face critical issues when it comes to generating manifold meshes. In the related works section, we first briefly discuss various indirect mesh generation methods. We then present detailed discussion on contemporary direct mesh prediction approaches which are closer to our approach. 

% There are several ways of representing 3D geometry such as voxel, point cloud, mesh and implicit functions which can be converted from one to another. Existing work on generating 3D meshes can be broadly categorized by the representation used. Methods that do not operate directly on meshes use several post-processing techniques to convert their representation to mesh. However, both the representation as well as post-processing methods for conversion to mesh can significantly affect the quality of the resultant mesh. In the related works section, we briefly discuss contemporary approaches that use representation other than meshes. Various techniques for converting them to a mesh. We then discuss in detail several methods that directly operate on meshes. 

\subsection{Indirect Mesh Prediction}
% Popular ways of representing a 3D geometry include voxel-based, point cloud, implicit function and mesh based representation.
% Instead of directly regressing a mesh, indirect approaches generate a mesh as a post-processing step.  

Indirect approaches tend to predict the 3D geometry as either a distribution of voxels\cite{voxel4}\cite{voxel5}\cite{voxel6} \cite{voxel1}\cite{voxel2}\cite{voxel3}\cite{HSP}\cite{Octtree}, point clouds\cite{PSG}\cite{foldingnet} or an implicit function representing signed distance from the surface. Both voxel and point set prediction methods struggle to generate high resolution outputs which later makes the iso-surface extraction tools ineffective or noisy\cite{AtlasNet}. 

% Early methods relied on voxelized representation but could not scale on more than $128^3$ resolution due to memory constraints\cite{voxel4}\cite{voxel5}\cite{voxel6} \cite{voxel1}\cite{voxel2}\cite{voxel3} unless some form of multi-resolution sparse data structure is used \cite{HSP}\cite{Octtree}. Recently point set generation methods\cite{PSG} have been popular as they give away connectivity information in favour of memory efficiency but they are also difficult to scale higher than an output resolution of 2500 points \cite{AtlasNet}. Moreover, Poission Surface Reconstruction which is used to extract mesh surface from point clouds is extremely sensitive to normal estimates and struggles to work with sparse points \cite{AtlasNet}. 
% Early methods have considered representing the surface of a 3D geometry as a distribution in voxel space \cite{voxel1}\cite{voxel2}\cite{voxel3}. However they struggle to achieve resolution higher than $128^3$ \cite{voxel4}\cite{voxel5}\cite{voxel6} unless some form of multi-resolution sparse data structure is used \cite{HSP}\cite{Octtree} but they are often too cumbersome to implement.

% Voxel grids are a natural extension of 2D pixel grids to 3D. They allow for easy retrofitting of standard 2D CNNs with 3D kernels, making it simpler to transfer the success of 2D deep learning to 3D. 
% However, due to the memory requirements, voxel-based approaches were limited to relatively small $32^3$ grids which resulted in very low resolution representations.
% While recent works\cite{voxel4}\cite{voxel5}\cite{voxel6} have pushed this limit to $128^3$, this has severely restricted depth of network architectures and training regimes. Some methods have also proposed to use a multi-resolution approach \cite{HSP}\cite{Octtree} but they are often too cumbersome to implement. 

% We can therefore conclude that the state-of-the-art voxel based surface generation fail to generate high-quality representation due to their memory requirements. 
% The most popular approach converting predicted voxel distribution into a mesh is by applying some variation of marching cube algorithm \cite{marching}. This however often results in meshes that are very low resolution and may not be closed or manifold. 
% Point set based representation of 3D surface, on the contrary are very cheap to store and operate since they give away the connectivity information. Recently point generation methods\cite{PSG} have been successfully developed using powerful point encoders \cite{pointnet}  \cite{pointnet++}. But their output resolution is often limited to a few thousand points, not enough make any dense predictions \cite{AtlasNet}. 

% They find wide applications in the robotics community since several sensors like Lidar and Radar actively capture 3D data that comes in as point clouds[citation needed]. However, a point set suffers from the problem of permutation invariance and lack of well defined neighbourhood. Recently, Qi et al. \cite{pointnet} solved the permutation invariance issue by applying a fully connected neural network to each point independently followed by a global pooling operation. In a subsequent work \cite{pointnet++} they proposed a hierarchical use of \cite{pointnet} to induce some sense of neighbourhood leading to improved performance.

% However, most of the point set generation methods have a fixed limit on the number of points they can generate which is at max 2500 [citation needed]. This is far from what is required to get any type of dense representation\cite{AtlasNet}. 
% Additionally, accurate surface normal estimation is required for applying the Poission Surface Reconstruction algorithm \cite{PSR} which is an ill-posed problem. 

% Unlike other approaches, converting a point cloud to mesh is very tricky. Most common way is to use Poission surface reconstruction (PSR) \cite{PSR} on the predicted point cloud, but this works only on dense point cloud (more than 100000 points) and is very sensitive to the quality of normal estimation \cite{AtlasNet}. 

% \subsection{Implicit Function Representation}
More recently, neural networks have been used to learn a continuous implicit function representing shape\cite{deepsdf}\cite{OccNet}\cite{ImplicitFields}. The idea is simply to feed a neural network with latent code and a query point (x-y-z) to predict the TSDF value \cite{deepsdf} or the binary occupancy of the point \cite{OccNet}\cite{ImplicitFields}. However, this approach is computationally expensive since in order to get a surface from implicit function representation, several thousands of points are required to be sampled which makes the process slow and time consuming at run time. Moreover, for shapes that have thin structures (like chair) implicit methods often fail to produce a singly-connected component.

% While some approaches still have a voxel based step in their pipeline which pose significant memory limitations, other methods have been able to circumvent this by training just with the sampled points\cite{disn}. Unfortunately, implicit representation comes with a huge memory cost as they are still required to predict the TSDF values of the entire voxel\cite{deepsdf}. To get the surface from implicit function representation, several thousands of points are required to be sampled which makes the process slow and time consuming at run time. Moreover, for shapes that have thin structures (like chair) implicit methods often fail to produce a singly-connected component.

% While implicit methods look promising, they suffer from several shortcomings. Firstly, they come with a huge memory cost as they are still required to predict the TSDF values of the entire voxel\cite{deepsdf}. Secondly, to get the surface from implicit function representation, several thousands of points are required to be sampled which makes the process slow and time consuming at run time. Lastly, for shapes that have thin structures (like chair) implicit methods often produce dis-connected components while the target shape is 1-connected. 

In spite varied levels of successes in terms of voxel, point cloud and implicit function representations, they all depend on the Marching Cube algorithm \cite{marching} for iso-surface extraction. While Marching Cube can be applied directly to the boundary voxel grids, point clouds first need to regress the iso-surface function using surface normal information. Note that implicit function representation learn to regress TSDF values per voxel instead and then perform extensive query to generate iso-surface based on a threshold $\tau$. Marching cube is essentially a look-up table for different triangle arrangement based on the classification of grid vertices $v_i \in \mathcal{V}$ as `inside' ($TSDF(v_i)\leq \tau$) and `outside' ($TSDF(v_i)\geq \tau$).  It should be noted however that marching cube does not guarantee \textit{manifoldness} of generated mesh \cite{marchingextended}\cite{marching33}\cite{marchingdualcountouring}. 

% \subsection{Converting various representations to mesh}
% The process of extracting a mesh representation from either a voxel, point-cloud and implicit function representation is quite tedious and often lack guarantees of \textit{manifoldness} of generated mesh. 

% Converting a voxel and implicit function representation follow a similar approach, apart from the fact that implicit function additionally need to do extensive query the TSDF for several thousands of points for each object and build a TSDF voxel. This process is therefore very slow and computation intensive. Once a voxel $\mathcal{V}$ of some arbitrary resolution in created, a threshold $\tau$ is chosen that gives the best iso-surface extraction on the validation set. Then some variant of the popular marching cube algorithm \cite{marching} is applied. Marching cube is essentially a look-up table for different triangle arrangement based on the classification of grid vertices $v_i \in \mathcal{V}$ as `inside' ($TSDF(v_i)\leq \tau$) and `outside' ($TSDF(v_i)\geq \tau$). It should be noted however that marching cube does not guarantee \textit{manifoldness} of generated mesh \cite{marchingextended}\cite{marching33}\cite{marchingdualcountouring}. 
% Conver
% The process of extracting a mesh from the implicit representation is also very tedious requiring time consuming query of several thousand points for a single object to provide descent shape and then applying marching cube. This process may not lead to a single connected mesh and the marching cube process doesnot guarantee manifold structure. However, marching cube does prevent self-intersection issue. 

\subsection{Direct Mesh Prediction}
A mesh based representation stores the surface information cheaply as list of vertices and faces that respectively define the geometric and topological information. Early methods of mesh generation relied on predicting the parameters of category based mesh models. While these methods output manifold meshes, they work only when parameterized manifold meshes are available for the object category. Recently some success has been made to generate meshes for a wide class of categories using topological priors \cite{AtlasNet} \cite{pixel2mesh}. Deep networks are used to update the vertices of initial mesh to match that of the final mesh. AtlasNet\cite{AtlasNet} uses chamfer distance applied on the vertices for training while Pixel2Mesh \cite{pixel2mesh} uses a coarse to fine deformation approach again using vertex chamfer loss. However, using a point set training scheme for meshes leads to severe topological issues and produced meshes are not manifold. Some recent works have proposed to use mesh regularizers like Laplacian\cite{pixel2mesh}\cite{geometrics}\cite{meshrcnn}\cite{3dn}, edge lengths\cite{meshrcnn}\cite{geometrics} and normal consistency\cite{meshrcnn} to constrain the flexibilty of vertex predictions however they suffer from \textit{regularizer's dilemma} as better geometric accuracy comes at a cost of manifoldness. 

% but it remains at best a heuristic only. They do not provide any guarantee of \textit{manifoldness} and infact makes the optimization process more difficult and leads to a loss in geometric accuracy\cite{meshrcnn}. 

In contrast to the aforementioned approaches, our approach leads to high resolution meshes with guaranteed \textit{manifoldness} across a wide variety of shape categories. The idea is similar to previous approaches \cite{AtlasNet}\cite{pixel2mesh}\cite{geometrics} based on deforming an initial ellipsoid by updating its vertices. However, instead of using explicit mesh regularizers, our approach uses NODE blocks to learn the deformation flow which as mentioned in section 2.2 implicitly discourage self-intersections to maintain the topology and therefore, guarantee \textit{manifoldness} of generated shape. The entire pipeline is end-to-end trainable without requiring any post-processing. 

